Automated Reinforcement Learning (AutoRL): A Survey and Open Problems

The combination of Reinforcement Learning (RL) with deep learning has led to a series of impressive feats, with many believing (deep) RL provides a path towards generally capable agents. However, the success of RL agents is often highly sensitive to design choices in the training process, which may require tedious and error-prone manual tuning. This makes it challenging to use RL for new problems, while also limits its full potential. In many other areas of machine learning, AutoML has shown it is possible to automate such design choices and has also yielded promising initial results when applied to RL. However, Automated Reinforcement Learning (AutoRL) involves not only standard applications of AutoML but also includes additional challenges unique to RL, that naturally produce a different set of methods. As such, AutoRL has been emerging as an important area of research in RL, providing promise in a variety of applications from RNA design to playing games such as Go. Given the diversity of methods and environments considered in RL, much of the research has been conducted in distinct subfields, ranging from meta-learning to evolution. In this survey we seek to unify the field of AutoRL, we provide a common taxonomy, discuss each area in detail and pose open problems which would be of interest to researchers going forward.

==> AutoRL Survey_axiv_v2_/storage/environment_design_storage.tex <==

\subsection{Environment Design}
\label{sec:envdesign}

Environment design is an important component for automating the learning in RL agents. From curriculum learning \cite{jiang2020prioritized, space_eimer_icml_21, spdrl_klink_nips_20, teacher_student_curri_matiisen_ieee_20, auto_curricula_sukhbaatar_iclr_18} to synthetic environment learning \cite{synth_envs_ferreira_metalearn_21a} and generation \cite{evolving_mario_gan_gecco_18} to combining curriculum learning with environment generation \cite{gpn_bontrager_arxiv_20, poet_wang_gecco_19, enhanced_poet_wang_icml_20, paired_dennis_nips_20}, the objective here is to speed up the learning for the RL agents through environment design. %In this section, we will explore literature that performs automated environment design (Section \ref{sec:auto_envdesign}) and describe papers that are manually designed but can be used to perform AutoRL (Section \ref{sec:man_envdesign_for_autorl}). 

%We begin with automated environment design in the next sub-section and then proceed to describe manually designed environments for AutoRL in the sub-section after.
% Model-Based RL (MBRL) which learns a model of the environment and is a core traditional RL technique can be viewed through the lens of speeding up learning (in terms of samples) on the real environment through environment design.
%  open-ended learning environments
% round robin paper too for curriculum?
% \rr{What about reward shaping? It learns a component of the env. R. Like MBRL it could also be viewed through the AutoRL lens but I don't think we'll include either of these as AutoRL.}

% \subsubsection{Automated Environment Design} 
% \label{sec:auto_envdesign}
% \textbf{Automated Environment Design} 
We organize algorithms performing Automated Environment Design according to the component of the environment (assumed to be a POMDP as defined in Section \ref{sec:preliminaries}) that they try to automatically learn.

% \paragraph{Transition function, $P$:}
% Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} proposed a method that learns a given target environment's transition function in order to train agents more efficiently. They framed this as a bi-level optimization problem and optimized the learnt environment (an NN) in an outer loop to maximize the reward of the agent in the inner loop. They showed that their \textit{synthetic environments} can not only serve as a more efficient proxy for expensive target environments, but that training on them can also reduce the number of training steps.

\paragraph{Reward function, $R$:} Zheng et al. \cite{learned_intrinsic_rewards_zheng_neurips_18} presented a bi-level optimization approach that learns reward shaping for policy gradient algorithms using a parameterized intrinsic reward function. The parameters of the agent are updated using gradient descent to increase the sum of intrinsic and extrinsic rewards. After this, the parameters of the intrinsic reward are updated using gradient descent to increase only the extrinsic rewards.
Hu et al. \cite{learn_reward_shaping_neurips_20} also presented a bi-level optimization approach which they term BiPaRS (and its variants). They use a PPO \cite{ppo_schulman_arxiv_17} agent in the inner loop. Further, they use meta-gradients with respect to the (state-action dependent) parameters of \textit{user-defined} reward shaping functions to learn helpful reward functions in the outer loop. Zou et al. \cite{reward_shaping_via_meta_learning_arxiv_19} proposed to meta-learn a potential function \cite{reward_shaping_ng_icml_99} prior over a distribution of tasks. Inspired by MAML \cite{maml_finn_icml17}, they try to adapt the meta-learned prior towards the optimal shaping function (which they derive to be equal to the optimal state-value function $V$). To learn the optimal V-values they use dueling-DQN. Konidaris and Barto \cite{autonomous_shaping_konidaris_icml_06} introduced a function that preserves value information between tasks and acts as the agent’s internal shaping reward. The input to this function is the part of the state space whose meaning doesn't change across tasks. This function can be used as the initial estimate for newly observed states and is further refined based on parts of the state space whose meaning does change across tasks. Snel and Whiteson \cite{multi_task_evolutionary_shaping_snel_gecco_10} used an evolutionary feature selection method and showed that this method chooses representations that are suitable for shaping and value functions. Their algorithm can find a shaping function in multi-task RL without pre-specifying a separate representation. Marthi \cite{automatic_shaping_and_decomposition_marthi_icml_2007} proposed automatically learning a shaped reward and a decomposed reward. Given a set of state and temporal abstractions, they create an abstracted MDP over the original MDP and learn the reward shaping using collected reward samples based on a mathematical formulation they derive.

Faust et al., \cite{faust2019evolving} investigate the effect of learning multi-objective inartistic reward over several RL algorithms and benchmarks. The results show that a) the utility of automated reward search correlates with the difficulty of the task, b) using simple sparse task objectives (e.g. maximize the distance travelled in MujoCo tasks where appropriate) as a fitness function over complex, hand-tuned Mujoco rewards leads close to identical results, and c) reward search is more likely to produce better policies that the HP search on a fixed training budget and with reasonable hyper-parameters. The study concludes with the best practices aimed at the practitioners: when training RL on complex tasks, first come up with reasonable hyper-parameters, then automate the inartistic reward search. Automate the intrestic reward search by formulating the reward as a parametrized features relevant to the problem (energy, safety, progress to the goal etc...), and use simple task objective (maximize the distance, reach a goal etc.) as a fitness function. Then search for the inartistic reward and corresponding policy with an evolutionary search.

\paragraph{Action Space, $\mathcal{A}$:} Simplifying an environment's action space can make training significantly easier and faster. The two main approaches used to accomplish this are repeating single actions in order to reduce the number of overall decision points or to construct a new action space entirely, composed of combinations of basic actions in macro actions or options.
While handcrafting has been common in action space augmentation, Sharma et al. \cite{learning_to_repeat} learned the number of repetitions for a given action alongside the action selection. Biedenkapp et al. \cite{temporl} presented an extension of the idea by conditioning the repetition prediction on the predicted action itself.
In automatic macro action discovery, Farahani and Mozayani \cite{macro_actions} showed that it is possible to combine actions into suitable macro actions by defining subgoals to be reached in the environment; this is achieved by partitioning its transition graph. 
Options are similar to macro actions, but instead of executing a macro action once, each option has its own intra-option policy that is followed until a termination function defers back to the agent \cite{options}. Bacon et al. \cite{ac_options} jointly learned both a policy across these options as well as the options themselves. The idea was also extended to learn options that are robust to model misspecification \cite{robust_options}.

\paragraph{Observation Space, $\mathcal{O}$:} Raileanu et al. \cite{ucb_drac} proposed using a UCB bandit to select an image transformation (e.g. crop, rotate, flip) and applying it to the observations. The augmented and original observations are passed to a regularized actor-critic agent which uses them to learn a policy and value function which are invariant to the transformation.

% \subsubsection{Manual Environment Design for AutoRL}
% \label{sec:man_envdesign_for_autorl}
% \textbf{Environment Design for AutoRL}


\paragraph{Multiple Components:} We discuss here approaches that change multiple components in the environment or the whole environment itself. Most notable here are curriculum learning approaches that usually modify the state space $S$ and the initial state distribution, $\rho$. As a result of modifying $S$, they naturally also change the $P$ and $R$ since these are functions with $S$ a component of their domains.

Wang et al. \cite{poet_wang_gecco_19} and Wang et al. \cite{enhanced_poet_wang_icml_20} proposed POET that generates new environments according to an environment encoding. The environments are automatically generated, either with random mutations \cite{poet_wang_gecco_19} or if the new environments create a significantly different ranking of existing agents \cite{enhanced_poet_wang_icml_20}. These methods of generating new environments are assumed to create a diversity of environments on which to train agents in a curriculum. Lee et al. \cite{quadrup_poetlike} applied the principle to controlling quadrupedal robots and found the robustness to increase significantly.

%\footnote{We categorize this under modification of the state space $S$ because the action space $A$, transition function $P$, reward function $R$ do not change and the observation space $\mathcal{O}$ and observation function $\Omega$ are only affected due to the change in the state space.}

Dennis et al. \cite{paired_dennis_nips_20} proposed PAIRED that also automatically generates new environments to create a curriculum. They used a fixed environment encoding. In contrast to \cite{poet_wang_gecco_19, enhanced_poet_wang_icml_20}, they employed a minimax regret formulation. They maintained an additional \textit{antagonist} agent (apart from the usual agent that they call the \textit{protagonist}). The regret is calculated as the difference between the performance of the protagonist and antagonist on sampled trajectories in sampled environments. They try to maximize this regret by sampling environments in which the antagonist outperforms the protagonist by as large a margin as possible. This keeps the environments still learnable for the protagonist since another agent (the antagonist, trained simultaneously with the protagonist) has already done much better on them and, thus, leads to better curricula. Gur et al., \cite{gur2021code}, propose Compositional Design of Environments (CoDE), a PAIRED extension for compostional tasks. CoDE's environment generative model builds a series of compositional tasks and environments tailored to the RL agent's skill level. CoDE archives that by working on a population of agents and observing their actual performance, in addition to regret. CoDE then adds an explicit difficulty loss, which encourages the generative model to tune the difficulty (how many sub-tasks) based on the observed competency of the agent, and use regret for fine-tuning of the environment and selection of the which design elements to use (sub-task selection). The resulting agent is able to generalize to space of $10^31$ tasks, induced with only 1500 sub-tasks.   

Extending the theoretical framework from PAIRED in a different direction, Jiang et al. \cite{jiang2021robustplr} showed that rather than learn to \emph{generate} new environments, it is also effective to \emph{curate} randomly sampled ones. Indeed, when doing so, it is possible to achieve similar robustness guarantees, without the need to learn an environment adversary which may be challenging in practice. This led to outperformance on the grid world tasks originally introduced by PAIRED, while also achieving strong performance on procedurally-generated car racing environments. 

Bontrager and Togelius \cite{gpn_bontrager_arxiv_20} also employed an environment generator and an actor-critic agent which work both cooperatively and adversarially to create a curriculum for the agent. They used automatically generated environments and human created environments in an equal proportion. The generator network tries to create environments that provide an appropriate level of challenge for the agent. The generator is an NN that learns to make content based on estimates by the critic. The generator uses the estimates to create environments which have an estimated value of 0 for the agent. So, initially when the agent has negative rewards, this results in the generator creating environments that would be easy for the agent but once the agent starts obtaining positive rewards the generator creates environments that still have 0 utility for the agent and thus makes it harder for the agent to do well. This process provides an implicit curriculum for the agent, creating more complex environments over time.


If the agent's goal is solving a specific task instead of being generally more robust, it can be supported by continually progressing a simple version of the task towards this goal in a curriculum \cite{narvekar-cl-survey-jmlr20}.
Progression is usually tied to how well the agent currently performs in order to keep the environment difficulty at an appropriate level.
OpenAI et al. \cite{openai-rubikscube} used this idea to use a robot hand to solve the Rubik's cube, by starting from an almost solved cube and gradually increasing the starting position complexity of both hand and cube as soon as the agent can solve the current state sufficiently well. 
Klink et al. \cite{spdrl_klink_nips_20} applied the sample principle to several physics simulation tasks, using value estimations as the progression criterion.
Value estimation approaches in general have been successful for RL because their approximation of an environment's challenge level is cheap to compute \cite{jian-spl-aaai15,zhang-vds-neurips20, space_eimer_icml_21}.
They are an important class in the starting state curriculum generation taxonomy proposed by \cite{woehlke-spl-aamas20}.
Student-teacher curriculum learning approaches can also create new task variations, e.g. by using GANs, although they only gradually increase the complexity of their distribution as the agent improves during training \cite{goal_gan,teacher_student_curri_matiisen_ieee_20,turchetta-neurips20}.
%such-gtn-pmlr20,
We can even induce a difficulty curve into environments that are immutable by using Self-Play to challenge agents with ever more difficult opponents \cite{auto_curricula_sukhbaatar_iclr_18,silva-ieee19}.


%Curriculum learning can also be applied for open-ended learning as shown in \cite{poet_wang_gecco_19,enhanced_poet_wang_icml_20}. Instead of moving towards a specific task configuration, the general environment complexity is simply increased in time with the agent's increased abilities.


%If the environment parameters are not well enough understood to manually generate challenging variations of a task, methods like \cite{paired_dennis_nips_20} can generate valid distributions across a given environment. 
%This could be compared to augmenting the agent's observations as in \cite{ucb_drac}.

Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} proposed a method that learns a given target environment's transition and reward functions in order to train agents more efficiently. They framed this as a bi-level optimization problem and optimized the learnt environment (an NN) in an outer loop to maximize the reward of the agent in the inner loop. They showed that their \textit{synthetic environments} can not only serve as a more efficient proxy for expensive target environments, but that training on them can also reduce the number of training steps. 
%Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} also learned a given target environment's using a bi-level optimization framework. 

% We describe \cite{autorl_learn_reward_nn_arch_chiang_ral19, Jaderberg859} in section \ref{sec:hybrid_approaches} as they employ not just environment design.

%While we have presented approaches that automatically learn $S$, $A$, $P$ and $R$, to the best of our knowledge there is no literature that tries to automatically learn $\mathcal{O}$ or $\Omega$. It might be useful to learn what observations increase the performance on an environment most while keeping the underlying state space fixed. For example, partial observability has been shown to improve generalization performance in grid-worlds \cite{paired_dennis_nips_20,transforms_zero_shot_ye_cog_20}.

\paragraph{Open Problems:} There are many varied approaches for environment design and it is unclear which of them leads to the biggest gains in performance. This raises the possibility of employing several of these methods in a single approach and studying which approach leads to the greatest gains in performance.
Furthermore, the research effort in automated environment design is not unified or focused on improving upon shared benchmarks. To further progress towards fully automated progression through environments, efforts like \cite{romac-tma-icml21} could be helpful in encouraging closer cooperation and better comparability.


 
However, differentiable architecture search has also been shown to have frequent catastrophic failure modes~\cite{Zela2020Understanding}, and multi-fidelity Bayesian optimization is a more robust approach that has already been used to optimize complex neural architectures for RL including both convolutional and recurrent layers~\cite{runge2018learning}.















==> storage/environment_design_storage.tex <==

\subsection{Environment Design}
\label{sec:envdesign}

Environment design is an important component for automating the learning in RL agents. From curriculum learning \cite{jiang2020prioritized, space_eimer_icml_21, spdrl_klink_nips_20, teacher_student_curri_matiisen_ieee_20, auto_curricula_sukhbaatar_iclr_18} to synthetic environment learning \cite{synth_envs_ferreira_metalearn_21a} and generation \cite{evolving_mario_gan_gecco_18} to combining curriculum learning with environment generation \cite{gpn_bontrager_arxiv_20, poet_wang_gecco_19, enhanced_poet_wang_icml_20, paired_dennis_nips_20}, the objective here is to speed up the learning for the RL agents through environment design. %In this section, we will explore literature that performs automated environment design (Section \ref{sec:auto_envdesign}) and describe papers that are manually designed but can be used to perform AutoRL (Section \ref{sec:man_envdesign_for_autorl}). 

%We begin with automated environment design in the next sub-section and then proceed to describe manually designed environments for AutoRL in the sub-section after.
% Model-Based RL (MBRL) which learns a model of the environment and is a core traditional RL technique can be viewed through the lens of speeding up learning (in terms of samples) on the real environment through environment design.
%  open-ended learning environments
% round robin paper too for curriculum?
% \rr{What about reward shaping? It learns a component of the env. R. Like MBRL it could also be viewed through the AutoRL lens but I don't think we'll include either of these as AutoRL.}

% \subsubsection{Automated Environment Design} 
% \label{sec:auto_envdesign}
% \textbf{Automated Environment Design} 
We organize algorithms performing Automated Environment Design according to the component of the environment (assumed to be a POMDP as defined in Section \ref{sec:preliminaries}) that they try to automatically learn.

% \paragraph{Transition function, $P$:}
% Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} proposed a method that learns a given target environment's transition function in order to train agents more efficiently. They framed this as a bi-level optimization problem and optimized the learnt environment (an NN) in an outer loop to maximize the reward of the agent in the inner loop. They showed that their \textit{synthetic environments} can not only serve as a more efficient proxy for expensive target environments, but that training on them can also reduce the number of training steps.

\paragraph{Reward function, $R$:} Zheng et al. \cite{learned_intrinsic_rewards_zheng_neurips_18} presented a bi-level optimization approach that learns reward shaping for policy gradient algorithms using a parameterized intrinsic reward function. The parameters of the agent are updated using gradient descent to increase the sum of intrinsic and extrinsic rewards. After this, the parameters of the intrinsic reward are updated using gradient descent to increase only the extrinsic rewards.
Hu et al. \cite{learn_reward_shaping_neurips_20} also presented a bi-level optimization approach which they term BiPaRS (and its variants). They use a PPO \cite{ppo_schulman_arxiv_17} agent in the inner loop. Further, they use meta-gradients with respect to the (state-action dependent) parameters of \textit{user-defined} reward shaping functions to learn helpful reward functions in the outer loop. Zou et al. \cite{reward_shaping_via_meta_learning_arxiv_19} proposed to meta-learn a potential function \cite{reward_shaping_ng_icml_99} prior over a distribution of tasks. Inspired by MAML \cite{maml_finn_icml17}, they try to adapt the meta-learned prior towards the optimal shaping function (which they derive to be equal to the optimal state-value function $V$). To learn the optimal V-values they use dueling-DQN. Konidaris and Barto \cite{autonomous_shaping_konidaris_icml_06} introduced a function that preserves value information between tasks and acts as the agent’s internal shaping reward. The input to this function is the part of the state space whose meaning doesn't change across tasks. This function can be used as the initial estimate for newly observed states and is further refined based on parts of the state space whose meaning does change across tasks. Snel and Whiteson \cite{multi_task_evolutionary_shaping_snel_gecco_10} used an evolutionary feature selection method and showed that this method chooses representations that are suitable for shaping and value functions. Their algorithm can find a shaping function in multi-task RL without pre-specifying a separate representation. Marthi \cite{automatic_shaping_and_decomposition_marthi_icml_2007} proposed automatically learning a shaped reward and a decomposed reward. Given a set of state and temporal abstractions, they create an abstracted MDP over the original MDP and learn the reward shaping using collected reward samples based on a mathematical formulation they derive.

Faust et al., \cite{faust2019evolving} investigate the effect of learning multi-objective inartistic reward over several RL algorithms and benchmarks. The results show that a) the utility of automated reward search correlates with the difficulty of the task, b) using simple sparse task objectives (e.g. maximize the distance travelled in MujoCo tasks where appropriate) as a fitness function over complex, hand-tuned Mujoco rewards leads close to identical results, and c) reward search is more likely to produce better policies that the HP search on a fixed training budget and with reasonable hyper-parameters. The study concludes with the best practices aimed at the practitioners: when training RL on complex tasks, first come up with reasonable hyper-parameters, then automate the inartistic reward search. Automate the intrestic reward search by formulating the reward as a parametrized features relevant to the problem (energy, safety, progress to the goal etc...), and use simple task objective (maximize the distance, reach a goal etc.) as a fitness function. Then search for the inartistic reward and corresponding policy with an evolutionary search.

\paragraph{Action Space, $\mathcal{A}$:} Simplifying an environment's action space can make training significantly easier and faster. The two main approaches used to accomplish this are repeating single actions in order to reduce the number of overall decision points or to construct a new action space entirely, composed of combinations of basic actions in macro actions or options.
While handcrafting has been common in action space augmentation, Sharma et al. \cite{learning_to_repeat} learned the number of repetitions for a given action alongside the action selection. Biedenkapp et al. \cite{temporl} presented an extension of the idea by conditioning the repetition prediction on the predicted action itself.
In automatic macro action discovery, Farahani and Mozayani \cite{macro_actions} showed that it is possible to combine actions into suitable macro actions by defining subgoals to be reached in the environment; this is achieved by partitioning its transition graph. 
Options are similar to macro actions, but instead of executing a macro action once, each option has its own intra-option policy that is followed until a termination function defers back to the agent \cite{options}. Bacon et al. \cite{ac_options} jointly learned both a policy across these options as well as the options themselves. The idea was also extended to learn options that are robust to model misspecification \cite{robust_options}.

\paragraph{Observation Space, $\mathcal{O}$:} Raileanu et al. \cite{ucb_drac} proposed using a UCB bandit to select an image transformation (e.g. crop, rotate, flip) and applying it to the observations. The augmented and original observations are passed to a regularized actor-critic agent which uses them to learn a policy and value function which are invariant to the transformation.

% \subsubsection{Manual Environment Design for AutoRL}
% \label{sec:man_envdesign_for_autorl}
% \textbf{Environment Design for AutoRL}


\paragraph{Multiple Components:} We discuss here approaches that change multiple components in the environment or the whole environment itself. Most notable here are curriculum learning approaches that usually modify the state space $S$ and the initial state distribution, $\rho$. As a result of modifying $S$, they naturally also change the $P$ and $R$ since these are functions with $S$ a component of their domains.

Wang et al. \cite{poet_wang_gecco_19} and Wang et al. \cite{enhanced_poet_wang_icml_20} proposed POET that generates new environments according to an environment encoding. The environments are automatically generated, either with random mutations \cite{poet_wang_gecco_19} or if the new environments create a significantly different ranking of existing agents \cite{enhanced_poet_wang_icml_20}. These methods of generating new environments are assumed to create a diversity of environments on which to train agents in a curriculum. Lee et al. \cite{quadrup_poetlike} applied the principle to controlling quadrupedal robots and found the robustness to increase significantly.

%\footnote{We categorize this under modification of the state space $S$ because the action space $A$, transition function $P$, reward function $R$ do not change and the observation space $\mathcal{O}$ and observation function $\Omega$ are only affected due to the change in the state space.}

Dennis et al. \cite{paired_dennis_nips_20} proposed PAIRED that also automatically generates new environments to create a curriculum. They used a fixed environment encoding. In contrast to \cite{poet_wang_gecco_19, enhanced_poet_wang_icml_20}, they employed a minimax regret formulation. They maintained an additional \textit{antagonist} agent (apart from the usual agent that they call the \textit{protagonist}). The regret is calculated as the difference between the performance of the protagonist and antagonist on sampled trajectories in sampled environments. They try to maximize this regret by sampling environments in which the antagonist outperforms the protagonist by as large a margin as possible. This keeps the environments still learnable for the protagonist since another agent (the antagonist, trained simultaneously with the protagonist) has already done much better on them and, thus, leads to better curricula. Gur et al., \cite{gur2021code}, propose Compositional Design of Environments (CoDE), a PAIRED extension for compostional tasks. CoDE's environment generative model builds a series of compositional tasks and environments tailored to the RL agent's skill level. CoDE archives that by working on a population of agents and observing their actual performance, in addition to regret. CoDE then adds an explicit difficulty loss, which encourages the generative model to tune the difficulty (how many sub-tasks) based on the observed competency of the agent, and use regret for fine-tuning of the environment and selection of the which design elements to use (sub-task selection). The resulting agent is able to generalize to space of $10^31$ tasks, induced with only 1500 sub-tasks.   

Extending the theoretical framework from PAIRED in a different direction, Jiang et al. \cite{jiang2021robustplr} showed that rather than learn to \emph{generate} new environments, it is also effective to \emph{curate} randomly sampled ones. Indeed, when doing so, it is possible to achieve similar robustness guarantees, without the need to learn an environment adversary which may be challenging in practice. This led to outperformance on the grid world tasks originally introduced by PAIRED, while also achieving strong performance on procedurally-generated car racing environments. 

Bontrager and Togelius \cite{gpn_bontrager_arxiv_20} also employed an environment generator and an actor-critic agent which work both cooperatively and adversarially to create a curriculum for the agent. They used automatically generated environments and human created environments in an equal proportion. The generator network tries to create environments that provide an appropriate level of challenge for the agent. The generator is an NN that learns to make content based on estimates by the critic. The generator uses the estimates to create environments which have an estimated value of 0 for the agent. So, initially when the agent has negative rewards, this results in the generator creating environments that would be easy for the agent but once the agent starts obtaining positive rewards the generator creates environments that still have 0 utility for the agent and thus makes it harder for the agent to do well. This process provides an implicit curriculum for the agent, creating more complex environments over time.


If the agent's goal is solving a specific task instead of being generally more robust, it can be supported by continually progressing a simple version of the task towards this goal in a curriculum \cite{narvekar-cl-survey-jmlr20}.
Progression is usually tied to how well the agent currently performs in order to keep the environment difficulty at an appropriate level.
OpenAI et al. \cite{openai-rubikscube} used this idea to use a robot hand to solve the Rubik's cube, by starting from an almost solved cube and gradually increasing the starting position complexity of both hand and cube as soon as the agent can solve the current state sufficiently well. 
Klink et al. \cite{spdrl_klink_nips_20} applied the sample principle to several physics simulation tasks, using value estimations as the progression criterion.
Value estimation approaches in general have been successful for RL because their approximation of an environment's challenge level is cheap to compute \cite{jian-spl-aaai15,zhang-vds-neurips20, space_eimer_icml_21}.
They are an important class in the starting state curriculum generation taxonomy proposed by \cite{woehlke-spl-aamas20}.
Student-teacher curriculum learning approaches can also create new task variations, e.g. by using GANs, although they only gradually increase the complexity of their distribution as the agent improves during training \cite{goal_gan,teacher_student_curri_matiisen_ieee_20,turchetta-neurips20}.
%such-gtn-pmlr20,
We can even induce a difficulty curve into environments that are immutable by using Self-Play to challenge agents with ever more difficult opponents \cite{auto_curricula_sukhbaatar_iclr_18,silva-ieee19}.


%Curriculum learning can also be applied for open-ended learning as shown in \cite{poet_wang_gecco_19,enhanced_poet_wang_icml_20}. Instead of moving towards a specific task configuration, the general environment complexity is simply increased in time with the agent's increased abilities.


%If the environment parameters are not well enough understood to manually generate challenging variations of a task, methods like \cite{paired_dennis_nips_20} can generate valid distributions across a given environment. 
%This could be compared to augmenting the agent's observations as in \cite{ucb_drac}.

Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} proposed a method that learns a given target environment's transition and reward functions in order to train agents more efficiently. They framed this as a bi-level optimization problem and optimized the learnt environment (an NN) in an outer loop to maximize the reward of the agent in the inner loop. They showed that their \textit{synthetic environments} can not only serve as a more efficient proxy for expensive target environments, but that training on them can also reduce the number of training steps. 
%Ferreira et al. \cite{synth_envs_ferreira_metalearn_21a} also learned a given target environment's using a bi-level optimization framework. 

% We describe \cite{autorl_learn_reward_nn_arch_chiang_ral19, Jaderberg859} in section \ref{sec:hybrid_approaches} as they employ not just environment design.

%While we have presented approaches that automatically learn $S$, $A$, $P$ and $R$, to the best of our knowledge there is no literature that tries to automatically learn $\mathcal{O}$ or $\Omega$. It might be useful to learn what observations increase the performance on an environment most while keeping the underlying state space fixed. For example, partial observability has been shown to improve generalization performance in grid-worlds \cite{paired_dennis_nips_20,transforms_zero_shot_ye_cog_20}.

\paragraph{Open Problems:} There are many varied approaches for environment design and it is unclear which of them leads to the biggest gains in performance. This raises the possibility of employing several of these methods in a single approach and studying which approach leads to the greatest gains in performance.
Furthermore, the research effort in automated environment design is not unified or focused on improving upon shared benchmarks. To further progress towards fully automated progression through environments, efforts like \cite{romac-tma-icml21} could be helpful in encouraging closer cooperation and better comparability.


 
However, differentiable architecture search has also been shown to have frequent catastrophic failure modes~\cite{Zela2020Understanding}, and multi-fidelity Bayesian optimization is a more robust approach that has already been used to optimize complex neural architectures for RL including both convolutional and recurrent layers~\cite{runge2018learning}.














